A Programming Language With a POMDP Inside

We present POAPS, a novel planning system for defining Partially Observable Markov Decision Processes (POMDPs) that abstracts away from POMDP details for the benefit of non-expert practitioners. POAPS includes an expressive adaptive programming language based on Lisp that has constructs for choice points that can be dynamically optimized. Non-experts can use our language to write adaptive programs that have partially observable components without needing to specify belief/hidden states or reason about probabilities. POAPS is also a compiler that defines and performs the transformation of any program written in our language into a POMDP with control knowledge. We demonstrate the generality and power of POAPS in the rapidly growing domain of human computation by describing its expressiveness and simplicity by writing several POAPS programs for common crowdsourcing tasks.

==> runningexample.tex <==
\section{Running Example}
We now consider a simple program that the following simple program that a crowdsourcing expert might use to improve a piece of text.
\begin{tabbing}
\noindent\texttt{(d}\=\texttt{efine} \texttt{(improve text}\\
\> \texttt{(c}\=\texttt{hoose} \\
          \>\>\texttt{(improve (dispatch crowd-improve 0 text))}\\
          \>\>\texttt{(dispatch return 0 text))}
\end{tabbing}
In this program, the \texttt{dispatch} call invokes a POMDP primitive action that hires a crowdworker to improve a piece of text and returns that piece of text. The program executes by choosing whether it should improve the piece of text and recurse, or terminate and return the piece of text. The argument \texttt{text} is bound to two values. The first value is a string and represents what the programmer cares about. The second hidden value $v \in [0,1]$ can be thought of as some measure of quality of the text. When these values are passed into the first \texttt{dispatch} call, a function is called to hire a crowdworker to improve the string, and the POMDP transition model is used on the hidden value to determine the hidden value of the improved string. Then, the new text and new hidden value are returned by \texttt{dispatch} and the program recurses. In this case, the POMDP model produces no observations, but if it did, the agent could use it to update its belief about the hidden value of the text. The POMDP model might also include a reward that represents the cost of hiring a worker. The second \texttt{dispatch} call uses the hidden value of the text in order to determine a reward, and it simply returns the text and its hidden value as is.


